Good things come in three: Generating SO Post Titles with Pre-Trained Models, Self Improvement and Post Ranking

Stack Overflow is a prominent Q and A forum, supporting developers in seeking suitable resources on programming-related matters. Having high-quality question titles is an effective means to attract developers' attention. Unfortunately, this is often underestimated, leaving room for improvement. Research has been conducted, predominantly leveraging pre-trained models to generate titles from code snippets and problem descriptions. Yet, getting high-quality titles is still a challenging task, attributed to both the quality of the input data (e.g., containing noise and ambiguity) and inherent constraints in sequence generation models. In this paper, we present FILLER as a solution to generating Stack Overflow post titles using a fine-tuned language model with self-improvement and post ranking. Our study focuses on enhancing pre-trained language models for generating titles for Stack Overflow posts, employing a training and subsequent fine-tuning paradigm for these models. To this end, we integrate the model's predictions into the training process, enabling it to learn from its errors, thereby lessening the effects of exposure bias. Moreover, we apply a post-ranking method to produce a variety of sample candidates, subsequently selecting the most suitable one. To evaluate FILLER, we perform experiments using benchmark datasets, and the empirical findings indicate that our model provides high-quality recommendations. Moreover, it significantly outperforms all the baselines, including Code2Que, SOTitle, CCBERT, M3NSCT5, and GPT3.5-turbo. A user study also shows that FILLER provides more relevant titles, with respect to SOTitle and GPT3.5-turbo.

==> commands.tex <==
\newcommand*{\ie}{i.e.,\@\xspace}
\newcommand*{\eg}{e.g.,\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}
\newcommand*{\etal}{et al.\@\xspace}

\newcommand{\nb}[2]{
	\fbox{\bfseries\sffamily\scriptsize#1}
	{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
}

\newcommand\RR[1]{\textcolor{blue}{\nb{Riccardo}{#1}}}
\newcommand\CDS[1]{\textcolor{red}{\nb{Claudio}{#1}}}
\newcommand\JDR[1]{\textcolor{orange}{\nb{Juri}{#1}}}
\newcommand\DD[1]{\textcolor{cyan}{\nb{Davide}{#1}}}
\newcommand\PTN[1]{\textcolor{green}{\nb{Phuong}{#1}}}

\newcommand*{\tool}{SERAPHINE\@\xspace}
\newcommand*{\HGF}{Hugging Face\@\xspace}

\newcommand*{\totPTM}{381,240\@\xspace}
\newcommand*{\notnullPTM}{140,149\@\xspace}
\newcommand*{\freqPTM}{135,915\@\xspace}
\newcommand*{\yamlonlyPTM}{8,482\@\xspace}
\newcommand*{\mixPTM}{TBD\@\xspace}



\newcommand*{\totTag}{40\@\xspace}
\newcommand*{\notnullTag}{40\@\xspace}
\newcommand*{\freqTag}{19\@\xspace}
\newcommand*{\yamlonlyTag}{19\@\xspace}
\newcommand*{\mixTag}{TBD\@\xspace}


\newcommand*{\mappedPTM}{TBD\@\xspace}
\newcommand*{\mappedTag}{TBD\@\xspace}



\newcommand{\iTODO}[1]{\todo[color=yellow!10, linecolor=black!50!yellow, inline]{\textbf{TODO:} #1}}
\newcommand{\RSPTD}[1]{\todo[color=blue!10, linecolor=black!50!blue, inline]{\textbf{SR1:} #1}}

\newcommand{\CDSTD}[1]{\todo[color=red!10, linecolor=black!50!red, inline]{\textbf{SR2:} #1}}

\newcommand{\MSTD}[1]{\todo[color=orange!10, linecolor=black!50!orange, inline]{\textbf{SR3:} #1}}

\newcommand{\change}[2]{\sout{\textcolor{red}{#1}}\textcolor{blue}{#2}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\lstdefinestyle{searchstringstyle}{
  basicstyle=\ttfamily\scriptsize,
%  breakatwhitespace=false,         
breaklines=true,                 
  captionpos=b,                    
%  keepspaces=true,                 
  numbers=none,                    
  numbersep=5pt,                  
  showspaces=false,                
  showstringspaces=false,
  showtabs=false,                  
  tabsize=2,
  frame=single
}


\newtcolorbox{shadedbox}{
drop shadow southeast,
%breakable,
enhanced jigsaw,
colback=white,
boxrule=0.80pt,
left=0.3em,
right=0.3em,
top=0.1em,
bottom=0.05em
}


\newcommand\revision[1]{\textcolor{blue}{#1}}

% research questions
%\newcommand{\rqfirst}{\textbf{RQ$_1$}: \textit{To what extent are the state-of-the art classifiers able to categorize PTMs using the model card?}}
\newcommand{\rqfirst}{\textbf{RQ$_1$}: \textit{How effectively can state-of-the-art classifiers categorize pre-trained models based on the information provided in their model cards?}}


%\newcommand{\rqsecond}{\textbf{RQ$_2$}: \textit{How can the proposed mapping help developers to select a proper PTM?}}
\newcommand{\rqsecond}{\textbf{RQ$_2$}: \textit{How can the suggested mapping contribute to assisting developers in the selection of an appropriate pre-trained model?}}




%\newcommand{\rqthird}{\textbf{RQ$_3$}: \emph{How the proposed mapping can help developers in selecting the proper PTM?}}
%\newcommand{\rqthird}{\textbf{RQ$_3$}: \emph{What are the best PTMs in terms of accuracy and energy consumption?}}

\newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\raw}\textcolor{blue}{\uline{#2}}}


 \newcommand*\circled[1]{\tikz[baseline=(char.base)]{\color{black} 
		\node[shape=circle,draw=black,fill=white!0!white,inner sep=.3pt] (char) {{{\texttt\textbf #1}}};}}



  %\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\color{black} 
%		\node[shape=circle,draw=cyan,fill=black!10!white,inner sep=.3pt] (char) {{{\texttt\textbf #1}}};}}




==> src/Discussion.tex <==
\section{DISCUSSION}~\label{sec:discussion}
 %AND THREATS OF VALIDITY

In this section, we discuss various implications ... Moreover, we also highlight the threats to validity of our findings.

\subsection{Implications}






\subsection{Threats to validity}

%\vspace{.1cm}
%\noindent
%$\rhd$~\textbf{Internal validity.} 

\begin{itemize}
    \item \textbf{Internal validity.} This concerns how well our evaluation resembles real-world scenarios. In the evaluation, we crawled data from \GH, and for the testing projects, we removed their real descriptions, and saved as ground-truth data. %This simulates a real development scenario where we need to recommend summary for repositories using their \RM. %adopted existing datasets~\cite{missing} manually curated and classified. The quality of the curated data depends very much on the evaluators' expertise. We anticipate that comments might be miss-classified, thus negatively impacting the overall prediction performance. 	
    \item \textbf{External validity.} This is related to the generalizability of the findings outside this study. %We attempted to mitigate the threats by evaluating \GS using different experimental configurations to simulate real-world scenarios. Since there exists no approach with the same purpose, \IT--a tool for generation of titles for bug reports--was chosen as the baseline. %for comparison. %For the comparison with the baseline, we used the original implementation published by the authors. 
%we extracted the results from the original paper and executed ... on the same datasets, using identical experimental settings. %Moreover, our proposed tool is applicable to other languages rather than Java, such as C++, Python, or R provided that there are proper tools to extract comments from source code to supply input for ...
    \item~\textbf{Construct validity.} This threat is related to the experimental settings to compare %\GS with \IT. To aim for a reliable comparison, we used the original implementation of \IT made available by its authors,\footnote{\url{https://github.com/imcsq/iTAPE}} keeping the internal design unchanged. Moreover, we tried to employ the same settings to experiment with both systems.
%\end{itemize}

\end{itemize}










% \subsection{Synergy of \tool and existing techniques}~\label{sec:combine}% 
% As discussed in Section~\ref{sec:rq2} and~\ref{sec:rq3}, we found that \tool excels in head and mid labels but performs worse than ZestXML in tail labels, which rarely happened.  In this section, we discuss the possibility of a synergistic approach of \LG and existing approach for better \GH topic recommendation. Particularly, we design a synergistic approach by combining top-3 predictions from ZestXML and top-5 predictions from \LG for the final top-8 predictions. The rationale behind this design is: (1) we observe that \LG and ZestXML show the optimal effectiveness on top-5 and top-3 predictions, respectively, and (2) we avoid bias on tail labels, which rarely happens and may harm performance. Table~\ref{tab:combine} illustrates the effectiveness of the synergistic approach compared to \LG and ZestXML.
% \begin{table}[h]
% \caption{The effectiveness (F1-score) of synergistic approach of ZestXML and \LG.}~\label{tab:combine}
% \begin{tabular}{l|cc|c}
% \hline
%      & \multicolumn{1}{l}{\textbf{ZestXML}} & \multicolumn{1}{l|}{\textbf{\tool}} & \multicolumn{1}{l}{\textbf{Synergistic approach}} \\ \hline
% \textbf{Head} & 0.340                        & \textbf{0.536}              & 0.532                         \\ 
% \textbf{Mid}  & 0.341                        & 0.473                       & \textbf{0.489}                \\ 
% \textbf{Tail} & 0.193                        & 0.079                       & \textbf{0.267}                \\ \hline
% \textbf{All}  & 0.337                        & 0.525                       & \textbf{0.526}                \\ \hline
% \end{tabular}
% \end{table}

% Overall, we can see that the synergistic approach outperforms ZestXML and \LG in mid and tail labels and only shows a slight decrease in performance in head labels. Consequently, the approach shows the best performance in whole labels. While the improvement is very marginal, we can see that this synergistic approach is more reliable than ZestXML and \LG as it offers consistent performance over different subsets of labels. We encourage future works to explore this direction for better \GH topic recommendation techniques. 

% \subsection{Threats to Validity} 
% \subsubsection{Internal Validity.} This threat refers to possible flaws in our experiments and implementations. We have carefully checked the correctness of our implementation. We also published our source code along with trained models~\cite{GitHubTopicRecSys} %at\footnote{} 
% and presented detailed hyper-parameters for the training of considered models in Section~\ref{sec:implementation}. Given these materials, other research can validate our results and findings. Therefore, we believe that there are minimal threats from this issue.  
% \subsubsection{Construct Validity.} This threat concerns the suitability of our evaluation. A source of these threats may stem from our evaluation metric. To minimize this threat, we employ well-known metrics, which are commonly used by prior studies~\cite{izadi2021topic,di2022hybridrec, lyu2023chronos, widyasari2023topic} for multi-label classification, including  Precision, Recall, and F1-score.

% \subsubsection{External Validity} This threat relates to the
% generalizability of our findings. Our experiments are conducted on the same dataset as prior work~\cite{widyasari2023topic}, crawled from \GH. This raises a concern about the external validity of our findings as they may not generalize beyond \GH repositories outside our dataset. However, we believe this threat is minimal as the dataset is exhaustively crawled from \GH and consists of a large number of data points, which ensure their diversity. 


==> src/Related_Work_backup.tex <==
\section{RELATED WORK} 
\label{sec:RelatedWork}
%\section{BACKGROUND AND RELATED WORK} 


This section introduces a brief overview on the background of Pre--trained Language Models (PLMs) along with their applications in Software Engineering and the state-of-the-art works for \SO post title generation.

\subsection{Pre-trained Language Models (PLMs)}
Deep learning has witnessed the successful application of the attention mechanism across diverse domains, ranging from image recognition, natural language processing (NLP), recommendation systems~\cite{zhao2020exploring,chaudhari2021attentive}.
The emergence of the Transformer architecture, introduced by Vaswani et al.~\cite{vaswani2017attention}, along with its adept utilization of attention mechanisms, has profoundly impacted the realm of NLP. This pivotal development has marked the onset of a new era for contemporary language representation models such as BERT~\cite{bert}, RoBERTa~\cite{roberta}, GPT-2~\cite{radford2019language}, BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}, and others.
These models share a commonality in employing transfer learning through pre-training, enabling them to acquire a comprehensive language representation from extensive unlabeled data, which can subsequently be fine-tuned for diverse downstream tasks~\cite{howard2018universal}. 
For instance, BERT~\cite{bert}, leveraging the encoder of the Transformer, proves to be a versatile Pre-trained Language Model (PLM) applicable in diverse downstream tasks like text similarity~\cite{tracz2020bert} and text classification~\cite{garg2020bae}. 
On the other hand, GPT-2~\cite{radford2019language}, relying on the Transformer’s decoder, excels in natural language generation problems~\cite{peng2020few}.
Lewis et al. introduced the BART model~\cite{lewis2020bart}, which incorporates both auto-regressive and bi-directional training objectives during pre-training, showcasing proficiency in diverse sequence-to-sequence tasks including document summarization, text generalization~\cite{akiyama2021hie}.
More recently, the T5 model~\cite{raffel2020exploring}, presented as a unified text-to-text PLM, consistently demonstrates state-of-the-art performance across tasks ranging from classification to generalization~\cite{zhuang2023rankt5}.
%PLMs for code
Apart from PLMs tailored for NLP tasks, research is increasingly focusing on Pre-trained Code and Language Models (PCLMs) to address programming language-related tasks. 
%like code summarization, API recommendation, code completion, and others. 
PCLMs, trained on code repositories, include diverse models such as CodeBERT~\cite{feng2020codebert}, PLBART~\cite{ahmad2021unified}, UnixCoder~\cite{guo2022unixcoder}, CodeT5~\cite{wang2021codet5}, and others.

Harnessing the substantial capabilities of PLMs and PCLMs, various studies have employed these models, achieving promising results in numerous Software Engineering (SE) tasks, including code summarization~\cite{ahmad2021unified,shi2022natural,zhou2022automatic}, program analysis~\cite{huang2022prompt}, code generation~\cite{liu2023refining}, to name a few. %and others.
Within these tasks, our study aligns most closely with the utilization of PLMs for code summarization~\cite{ahmad2021unified,shi2022natural,zhou2022automatic} and natural language-based text summarization in SE tasks, such as GitHub dialog summarization~\cite{fan2023dialog} and pull-request title generation~\cite{irsan2022autoprtitle,zhang2022automatic}.
Fan et al.~\cite{fan2023dialog} proposed ADSum, utilizing a fine-tuned T5 model to analyze GitHub discussion posts and generate summaries for annotators. 
They introduced the prompt-tuning technique to leverage few-shot annotated data for producing high-quality summarization of the dialog.
Zhang et al.~\cite{zhang2022automatic} have introduced the task of automatic generation of pull request titles for GitHub repositories using pre-trained baseline models, such as BERTSumExt~\cite{liu2019text}, BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}.% and others. 

%to the specialized field of software engineering~\cite{vaswani2017attention,von2022validity,li2023pre}.
%Pre-trained Language Models (PLMs), exemplified by BERT~\cite{bert}, RoBERTa~\cite{roberta}, BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}, and others, rely typically on the Transformer architecture, pioneered by Vaswani et al.~\cite{vaswani2017attention}, particularly leveraging attention mechanisms for their effectiveness and success in various research domains.
%These models are trained on extensive datasets, enabling them to grasp both the syntax and semantics of natural languages.






\subsection{Title Generation for \SO posts}
\SO (SO) serves as a widely used Question-Answering platform where software developers can seek solutions to programming-related queries. Mondal et al.~\cite{mondal2021early} highlighted that an increasing number of open questions on SO remain unanswered, partially attributed to the suboptimal quality of the question expression. Numerous research endeavors have been dedicated to addressing this issue, with a specific focus on crafting high-quality question titles~\cite{gao2021code2que,zhang2022improving,liu2023automated,zhang2023diverse,liu2022sotitle,zhou2023qtc4so}.
These investigations predominantly revolved around generating question titles by analyzing the content of SO posts, including problem descriptions and code snippets.

%code snippets to title - code summarization
Initial studies in this domain depended solely on code snippets for generating question titles, aligning closely with the code summarization task~\cite{tang2022ast,cheng2022keyword,shi2022natural,zhou2022automatic}. 
The concept of code summarization was initially conceived as a specialized Programming Language-to-Natural Language translation task, employing the sequence-to-sequence architecture within the encoder-decoder paradigm~\cite{ahmad2021unified}.
Building on this foundation, Gao et al.\cite{gao2021code2que} introduced Code2Que to generate Stack Overflow titles. This model employs bi-directional LSTMs, coupled with an attention mechanism, to encode the sequence of code tokens into hidden states, subsequently decoding them into concise question titles in natural language. 
This method also incorporated two conventional Natural Language Processing (NLP) techniques. It implemented a coverage mechanism~\cite{tu2016modeling} to mitigate word repetition issues and a copy mechanism~\cite{gu2016incorporating} to address out-of-vocabulary challenges.
Despite Code2Que exhibiting promising performance, LSTMs may struggle to handle long-range dependencies, leading to challenges in capturing the semantic meaning of the entire source code.
The most recent research efforts seek to harness the extensive dataset for pre-training language models and then fine-tuning for a specific task, resulting in state-of-the-art achievements, particularly in code summarization~\cite{ahmad2021unified,guo2022unixcoder} and SO post title generation~\cite{zhang2023diverse}.
Ahmad et al.~\cite{ahmad2021unified} introduced the Transformer model to tasks related to programming languages such as code summarization, code generation and code translation.
They proposed PLBART with the use of pairwise position encoding to capture the long-range dependencies among code tokens.
Subsequent studies focus on introducing multilingual representation models tailored for programming languages, as exemplified by UnixCoder~\cite{guo2022unixcoder}, CodeT5~\cite{wang2021codet5}.
Zhang et al.~\cite{zhang2023diverse} introduced M3NSCT5, fine-tuning the CodeT5 model to translate code sequences into relevant titles for Stack Overflow posts. 
However, the lack of context around code snippets can lead to the same code snippets being associated with different titles, introducing ambiguity. 
In addressing this, M3NSCT5
%their method \textbf{DAVIDE: WHICH ONE?} 
emphasizes diversifying generated texts using Nucleus Sampling strategy~\cite{holtzman2019curious} and Maximal Marginal Ranking~\cite{yang2021maximizing}, providing users with a selection of titles for a given code snippet.
While our approach shares the aspect of producing multiple candidates during the inference stage, our primary goal differs – we aim to identify the most relevant title aligned with the input question description and code snippets.

%(description + code snippets) to title - abstractive text summarization
Zhang et al.~\cite{zhang2022improving} showed that incorporating both the problem description and code snippets contributes to clarifying the context, enhancing the clarity, and improving the completeness of question titles.
Recent studies in the realm of code summarization also proved that the inclusion of additional information, such as API documentation~\cite{hu2018summarizing}, source code comments~\cite{wei2020retrieve}, alongside the source code, has demonstrated improved performance compared to relying solely on the source code.
Pre-trained Language Models with the ability of multi-modal input modelling are typically adopted in these studies.
Zhang et al.~\cite{zhang2022improving} have introduced CCBERT, which leverages the pre-trained CodeBERT model~\cite{feng2020codebert} to parse bi-modal contents (i.e., problem description and code snippets), incorporated with the copy mechanism~\cite{gu2016incorporating} to handle rare tokens.
Liu et al.~\cite{liu2022sotitle} also incorporate multi-modal modeling in their approach, presenting SOTitle for generating Stack Overflow post titles.

SOTitle was constructed upon the pre-trained T5 model~\cite{raffel2020exploring}, aiming to establish a unified model for concurrent training across multiple programming languages. Subsequent research endeavors have adopted this input representation approach for Stack Overflow post title generation~\cite{zhang2023diverse,liu2023automated,zhou2023qtc4so}.
Instead of creating new titles for SO posts, Liu et al.~\cite{liu2023automated} focused on reformulating question titles through the analysis of modification logs on the Stack Overflow platform.
The proposed QETRA model also employs the pre-trained T5 as the backbone model to learn the title reformulation patterns from the extracted title modification logs.
In contrast to previous research, QETRA employs both the question body (comprising code snippets and problem description) and the question titles provided by users to suggest candidate reformulated titles.
Another task closely related to the generation of Stack Overflow post titles is the completion of question titles.
Zhou et al.~\cite{zhou2022automatic} introduced QTC4SO, an innovative approach for generating Stack Overflow post titles from bi-modal post contents and incomplete titles. Utilizing the pre-trained T5 model, QTC4SO learns potential title completion patterns and incorporates a multi-task learning strategy to leverage meaningful information from various programming languages.




%paragraph{The Application of PLMs in Software Engineering}




% This section introduces a brief overview of the background and related works. First, we present recent studies on the problem of topic recommendation for GitHub repositories. Subsequently, we delve into Large Language Models (LLMs) and their applications for Software Engineering Tasks.

% \subsection{Topic Recommendation for GitHub Repositories}
% \GH topic recommendation is related to %the problem of 
% suggesting relevant topics to repositories on GitHub. In this section, we first recall state-of-the-art techniques for this topic, and then introduce our problem formulation.

% \subsubsection{State-of-the-arts.} Recent approaches in \GH topic recommendation falls into two main categories.

% \vspace{1mm}

% \noindent \textbf{Probability-based Recommendation:} Recommenders based on probability \cite{di2020multinomial, di2022hybridrec, di2020topfilter}, formulate this problem as \textit{multi-class classification} and then employ algorithms, such as Multinomial Naïve Bayesian~\cite{di2020multinomial} to output probability that indicate how likely a topic belong to \GH repository. Particularly, given these probabilities, these techniques rank topics to offer recommendations. In this work, we exclude probability-based techniques such as MNBN~\cite{di2020multinomial} as they have been proven to be less effective than the multi-label-based approaches described below. 

% \vspace{1mm}

% \noindent \textbf{Multi-label Classification:} In contrast to the aforementioned approaches, Izadi et al. \cite{izadi2021topic} recently formalized the GitHub repository topic recommendation task as a \textit{multi-label classification} problem \cite{herrera2016multilabel}. They conducted empirical studies exploring various combinations of (1) document representation and (2) multi-label classification. Their experiments highlighted Logistic Regression with TF-IDF embeddings as the superior combination for topic recommendation, outperforming probability-based recommendation approaches~\cite{izadi2021topic}. Widyasari et al.~\cite{widyasari2023topic} further explores this direction by considering user-defined topics, formulating this problem as an extreme multi-label classification problem. Then, they conducted an exploration study to examine the effectiveness of XML techniques and found that ZestXML~\cite{zeroshotxml} is the best-performing approach in suggesting \GH topics. 

% \subsubsection{Problem Formulation.}
% In this work, we focus on \GH featured topics, which are
% carefully designed and maintained by \GH and its community, following Izadi \etal~\cite{izadi2021topic} as user-defined \GH topics may be noisy and of low quality. However, as rare topics may be still correct and important, we follow Widyasari~\cite{widyasari2023topic} to not remove them. This allows us to ensure both the quality of our dataset and the reliability of the recommendation systems produced in this study. As a result, we obtained a dataset of 665 unique topics (see Section~\ref{sec:dataset}). %Therefore, w
% We formulate our task as a multi-label classification problem, formally explained as follows. %We formally formulate the problem as follow:

% \vspace{1mm}

% \noindent \textbf{Prior Knowledge.} A labelled dataset $\mathcal{D} = (\mathcal{G}, \mathcal{T}, \mathcal{M})$, where $\mathcal{G}$ is set of GitHub repositories and $\mathcal{T}$ is set of featured topics. $\mathcal{M}$ is a mapping from $\mathcal{G}$ to set of subsets of $\mathcal{T}$, where $\mathcal{M}(g) \subseteq \mathcal{T}$ is the set of topics for a GitHub repository $g$.

% \vspace{1mm}

% \noindent \textbf{Input.}  A new (unlabelled) dataset $\mathcal{D}_{new} = (\mathcal{G}_{new}, \mathcal{T}_{new})$ where $\mathcal{G}_{new} \neq \mathcal{G}$ is a set of  repositories and $\mathcal{T}_{new} \supseteq \mathcal{T}$ is set of labels. We consider the repositories' descriptions and README files in this study.

% \vspace{1mm}

% \noindent \textbf{Output.} A mapping $\mathcal{M}_{new}$ from $\mathcal{G}_{new}$ to set of subsets of $\mathcal{T}_{new}$ such that $\mathcal{M}_{new}(g) \subseteq \mathcal{T}_{new}$ is the set of labels for each repository $g \in \mathcal{G}_{new}$.


% \subsection{Pre-trained Language Models}
% Pre-trained Language Models (PTMs) ~\cite{bert, roberta, lewis2020bart, electra} become popular in many domains including Natural Language Processing and Software Engineering thanks to their remarkable capabilities. These models are commonly built based on a Transformer architecture~\cite{vaswani2017attention} and trained on a massive amount of data, allowing them to learn and capture both the syntax and semantics of human language. Given these capabilities, PTMs showed excellent performance in extracting semantic features from textual data and great promise to be fine-tuned for tasks that they were not initially trained for~\cite{min2023recent, yang2022aspect, hou2023large, nguyen2023multi, zhang2020sentiment}.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.69\textwidth]{img/TopicRecommend.pdf}
%     \caption{Overall workflow of \tool.}
%     \label{fig:overview}
% \end{figure*}

% Inspired by these successes, PTMs have been widely adopted in Software Engineering tasks such as code generation~\cite{wang2021codet5, liu2023refining, chen2021evaluating}, program analysis~\cite{huang2022prompt, le2022autopruner, chow2023beware}, and program understanding/reasoning~\cite{ahmed2022few, le2023invalidator, wang2022bridging}. Among these tasks, the applications of PTMs for Natural Language-based Software Engineering (NLBSE) tasks are most closely to our study. Zhang \etal~\cite{zhang2020sentiment} investigated the capabilities of PTMs on sentiment analysis for Software Engineering. He \etal~\cite{he2022ptm4tag} showed the potential of PTMs for recommending tags in Stack Overflow posts. Wang \etal~\cite{wang2021well} proposed the use of PTMs for labeling \GH issues. Messaoud ~\cite{messaoud2022duplicate} applied PTMs for detecting duplicated bug reports. PTMs have been also applied to various other NLBSE tasks such as requirement classification~\cite{luo2022prcbert}, README simplication~\cite{gao2023evaluating}, Software Q\&A~\cite{xu2023we, yang2022answer}. Different from these works, our work delves into the problem of \GH Topic Recommendation. We also investigate challenges, \eg long-tailed distributions for applying PTMs on these tasks, and propose effective mechanisms for handling these challenges. 

% % First paragraph: Introduce about LLM and its capabilities

% % Second paragraph: Present applications of LLM for SE Tasks, e.g., Technical Q&A, Code Summarization, Code Generation, ...
